Automatic Retrieval-augmented Generation of 6G Network Specifications for Use Cases

6G Open Radio Access Networks (O-RAN) promises to open data interfaces to enable plug-and-play service Apps, many of which are consumer and business-facing. Opening up 6G access lowers the barrier to innovation but raises the challenge that the required communication specifications are not fully known to all service designers. As such, business innovators must either be familiar with 6G standards or consult with experts. Enabling consistent, unbiased, rapid, and low-cost requirement assessment and specification generation is crucial to the O-RAN innovation ecosystem. Here, we discuss our initiative to bridge service specification gaps between network service providers and business innovators leveraging Large Language Models (LLMs). We first review the state-of-the-art and motivation in 6G plug-and-play services, capabilities, potential use cases and LLMs. We identify an ample innovation space for hybrid use cases that may require diverse and variational wireless functionalities across its operating time. We show that the network specification can be automated and present the first automatic retrieval-augmented network service specification framework for 6G use cases. To enable public acceptance and feedback, a website interface is published for the research and industrial community to experiment with the framework. We hope this review highlights the need for emerging foundation models for this area and motivates researcher engagement and contribution to the community through our framework.

==> reviewer_comments.tex <==
Automatic Retrieval-augmented Generation of 6G Network Specifications for Use Case
[IEEE Comm Mag] – Reviewer Comments
% Not sure what format the submission system takes. so I'm changing this to pure text for maximal compatibility.

====================================

Reviewer 1

====================================

Comment 1.1
---------------------
The problem to solve is not clearly articulated. If we provide LLM and RAG to bridge the gap between network innovators who build AI apps and network providers who deploy 6G network and will own use cases, how the RAG can help versus specification in 3GPP and the ORAN-like specs.

Reply 1.1
---------------------
Dear reviewer, thank you for the question. Indeed, our framework is proposed to mimic the role of an expert 6G consultant with access to technical specifications and expert experience primarily for innovators of networked use cases. The role of the LLM is to offer cheap and wider access to small innovators who cannot afford telecom consultants or to give them early ideas on what is required before discussing details with consultants. In this review, we believe this is one of the earlier works to try and tackle this problem. We have a feedback plan to quantify the time-saving and cost-saving compared to reading specifications and consulting with telecom experts in the future (see revised Section V).

In addition, specifications in 3GPP and O-RAN Alliance have inherent limitations (see revised Section III.B Limitation 4). First, it is unlikely for the documents to cover all concrete use cases as they can have hybrid or evolving specification requirements. Second, most of the specification documents are network service provider-oriented, such as use case 2 (Flight Path-Based Dynamic UAV Radio Resource Allocation) and use case 3 (Radio Resource Allocation for UAV Application Scenario) discussed in the document "O-RAN Use Cases Detailed Specification 14.0" by O-RAN Alliance (https://specifications.o-ran.org/specifications), which focus on the design of O-RAN RAN Intelligent Controller instead of the specification descriptions from the use case innovator (e.g., UAV developer)'s point of view. Third, the specification documents cannot provide live information on the available networking resources to the use case innovators. Hence, we believe our framework, built to consolidate knowledge from specification documents, community-contributed use cases and live network data, will prove beneficial and irreplaceable to both network service providers and use case innovators.


Comment 1.2
---------------------
Also, what will be the risk that RAG brings information that can mislead rather than lead the network innovators and share useful information.

Reply 1.2
---------------------
Indeed, publicly available LLMs (e.g., GPT-4) by themselves may extract incorrect knowledge due to misinformation on the wider internet (see revised Section III.A). In our case, we did not retrain an LLM but instead augmented GPT-4 with a RAG knowledge database populated by knowledge indexed from verified sources, such as official 5GPP, O-RAN, and ETSI specification documents provided by the network service providers and validated use cases contributed by the community. This will reduce the risk of misinformation. However, the knowledge base here is relatively limited.
In the next phase, we plan to open up an upload portal for the community to upload peer-reviewed IEEE papers, diversifying the knowledge base. Every piece of knowledge saved in the knowledge database for RAG will be viewable, and commentable by the community (see revised Fig.3 Phase 2). These combined approaches limit the level of misinformation.


 1. Please see above.

\textbf{4.One more thing is on the developed framework, it is hard to tell what it is in terms of tangible thing. Are the authors building a RAG or using an open source solution? how this RAG is being populated with Data? what does this work offer to the community today and who will be the consumer/user of the framework?

Reply 1.3
---------------------
Dear reviewer, we have deleted the old Fig. 2 and added a new Fig. 1 in the Introduction Section, presenting a functional overview of the proposed platform focusing on how the targeted users, i.e., network service provider and networked use case innovator, interact with the platform. The platform implementation is comprised of two main components, the full-stack website interface and the RAG knowledge database. More details on the usage of the platform can be found in the revised Fig. 3 and Section IV.

The RAG pipeline is built with the open-source LlamaIndex framework (one of the most popular RAG frameworks) and the knowledge database is powered by the publicly available MongoDB Atlas Database (see revised first paragraph of Section IV). The knowledge in the database mainly consists of the use case data formatted according to the Use Case Ontology and user feedback (votes and comments). Constructing such a customized knowledge database with LlamaIndex is straightforward following tutorials on the LlamaIndex official website.


====================================

Reviewer 2

====================================

Comment 2.1
---------------------
Really appreciate you exploring the very timely topic of ORAN innovation platform based open ecosystem and how to close the co-ordination and collaboration gaps. Well written manuscript with tutorial nature and conceptual novelty.

As you wrote, the way network services are being developed, delivered, and utilized in the 6G era will be increasingly built on different aspects of the open network architecture. In particular, the introduced exposure to network data, service, and transaction capabilities as northbound service APIs, operation APIs, and network APIs will allow the developer community to create value via access to network capabilities while providing the mobile network operators (MNOs) opportunities to capture value from their own network capabilities.

To further strengthen the tutorial nature and the completeness of your manuscript should be glad if in addition to ORAN you could discuss the recent system architecture framework developments among other standardization bodies and industry forums such as 3GPP, TeleManagement Forum (TMF) and Linux foundation. E.g., Linux foundation’s open source CAMARA project collaborates with the Groupe Speciale Mobile Association (GSMA) to define, align, and publish interface requirements. See e.g., the following refs:

5G PPP Software Network WG, “Network Applications: Opening up 5G and Beyond Networks,” 2023.
3GPP CAPIF “Common API Framework”.
TM Forum, “TMF IF1167 – ODA Functional Architecture”, 2020.
CAMARA, “The Linux Foundation Telco Global API Alliance project,”. available online: https://camaraproject.org/

Reply 2.1
---------------------
Dear reviewer, this is a good point. In addition to indexing the pre-loaded specification documents provided by the network operators, we can dynamically pull in the knowledge of the available network resources in the RAG database through the APIs published by the network itself. We have embedded the suggested references in the paper and added appropriate text to contextualise your helpful suggestions (see revised Fig. 1, Fig. 3 Phase 3 and Section IV.C).


====================================

Reviewer 3

====================================

Comment 3.1
---------------------The paper introduces an automatic retrieval-augmented specification generation (RAG) framework to translate 6G use case descriptions into specifications. In this regard, the authors initiate a crowd-sourced knowledge database for 6G use cases with their corresponding specifications and implement an extensible user interface for stakeholders to perform automatic use case extraction and specification generation powered by a RAG architecture. The authors argue that this approach would bridge the gap between network service providers and business innovators.

The paper is well-written and organized, but the shared website user interface (https://ntutangyun.github.io/llm\_6g\_frontend) is not rendered.

Reply 3.1
---------------------
Dear reviewer, sorry for the unfortunate experience. The front end is hosted by Github, which should render correctly unless the reviewer cannot access the Github pages. There was an electricity outage that lasted for a few days during the review period which affected the back-end server. The problem is resolved and please give it a try again.


Comment 3.2
---------------------
The authors settle for the top-2 matched use cases, which raises a question about the scalability of the embedding, querying and retrieval pipeline (Fig. 5). How would techniques such as PCA, t-NSE or clustering help improve speed, accuracy and scalability?

Reply 3.2
---------------------
The 6G use cases and other knowledge saved in the knowledge database will increase and diversify over time. Indeed, knowledge scalability may become an issue as formal specification is intermixed with imaginative design solutions in the future. The number "2" here is a hyper-parameter of the retrieval process in RAG indicating the amount of retrieved knowledge for prompt augmentation. Ideally the larger the number is, the more references the LLM gets for generation and thus the better the results. However, the context length for any LLMs is limited now; longer prompts will incur higher costs (in terms of tokens) and may even confuse the LLM. By PCA, t-SNE, or clustering, we understand the reviewer is suggesting that we first retrieve more knowledge, and then distil or summarize the key points for prompt augmentation. This is a common practice in RAG pipeline design and has the potential to improve scalability, which is briefly mentioned in the last paragraph ("Advanced prompt engineering ..., filtering, ...") of Section IV.B. Nevertheless, a decision on this hyper-parameter still has to be made and thus we have changed the label top-2 to top-n for clarification (see revised Fig. 5).


Comment 3.3
---------------------
and would fine-tuning the LLM with a higher number of matched use cases lead to any substantial improvement of specification?

Reply 3.3
---------------------
Fine-tuning is shown to have the potential to improve performance, but some argue that fine-tuning may also lead to performance degradation as it may impact the trained knowledge. We plan to fine-tune a local LLM in the future and publish it to the community for free once we gather sufficient use cases (see revised Section V State I).


Comment 3.4
---------------------
The paper lacks metrics to quantitatively characterize the LLM performance, and justify the use of an LLM over another. The authors could compare e.g., hallucination or BLEU scores.

Reply 3.4
---------------------
The platform is built with the open-source RAG framework LlamaIndex (see first paragraph in revised Section IV) which is compatible with open-source RAG evaluation tools such as Ragas (https://docs.ragas.io/en/stable/). However, existing quantitative metrics such as hallucination or BLEU scores only evaluate the RAG performance (of different LLMs) in terms of retrieval-wise accuracy according to the indexed documents in the knowledge database; and the retrieval-wise accuracy of the generated specifications (e.g., latency, reliability or security) does not necessarily mean optimal performance after deployment as the indexed knowledge can be obsolete or sub-optimal. To address this, we propose two solutions: 
- in the current stage, we open a voting and comment interface on the website to allow the community to feedback on the generated specifications. All the (up and down) voting results and comments are publicly viewable on the website (see revised Fig. 3 Phase 2). 
- meanwhile, we are extending the feedback loop into the use case deployment stage and plan to explore evaluation approaches for operation-wise accuracy (see revised Section V Stage IV).


Comment 3.5
---------------------
How would the proposed framework benefit from the standardization bodies (such as 3GPP and O-RAN alliance) specifications/technical reports data to further fine-tune the LLM?

Reply 3.5
---------------------
Part of the knowledge in the RAG database is extracted from specifications provided by the network operator, and it is up to the network operator to choose standards from the 3GPP or O-RAN Alliance for knowledge indexing during the initialisation phase. Fine-tuning the LLM will leverage not only the specification documentation but also the user-contributed use cases and even user comments collected from the website (see revised Fig. 3, Section IV.C and Section V Stage I.)

On the reverse, we can also highlight what knowledge vectors are most appreciated through the community feedback mechanism, which can advise the standard bodies on usage (see revised Fig. 3 Phase 3).


====================================

Reviewer 4

====================================

Comment 4.1
---------------------
RAG (Retrieval-Augmented Generation) has proven effective in addressing the issue of 'AI hallucination' commonly found in large language models (LLMs). Combining RAG with LLMs creates a powerful tool for next-generation cellular systems like 6G. This integrated system can handle tasks such as automatic network specification and more. The paper proposes using such a system to generate detailed network specifications for specific 6G use cases.
Adding a separate section to provide a tutorial on LLM

Reply 4.1
---------------------
Dear reviewer, thank you for the suggestion. We have revised Section III. A with new introductory content covering LLMs' input and output, the training behind the remarkable performance, common usage scenarios, the SOTA LLMs and why RAG is adopted. 


Comment 4.2
---------------------
I believe it is important to discuss open-source tools from NVIDIA and others in this context to show what is the missing gap that the novelty of the paper is addressing. https://github.com/NVIDIA/GenerativeAIExamples/tree/main/experimental/oran-chatbot-multimodal

Reply 4.2
---------------------
The O-RAN chatbot by Nvidia and another work "Telco-RAG: Navigating the challenges of Retrieval-augmented language models for Telecommunications" (on Arxiv) are both applications or customization of the RAG pipelines in the telecom domain. They focus on answering factual questions about the telecom documents. Our framework takes a step further by distilling relevant knowledge from the documents, community contributions and potentially live network data to assist in the use case innovation and network optimization (see revised first paragraph of Section V).


Comment 4.3
---------------------
While I appreciate the associated web page as a service to show the catalog for different 6G use cases and corresponding network specification, I missed any open source contribution part for the community.

Reply 4.3
---------------------
The full-stack solution is still in the prototype phase and we will open-source publicly both frontend and backend for the community to contribute once the code base is stable and mature enough. However, we are happy to share and discuss the current implementation when requested privately through our emails.


Comment 4.4
---------------------
sec II, C  how the proposed method can address the mentioned limitation 3

Reply 4.4
---------------------
All the knowledge, including community-contributed use cases, feedback and those distilled from documents is made publicly available on the website by default. The knowledge especially the list of use cases with networking specifications will provide valuable references when the network service provider is designing the internal RIC (e.g., xApp or rApp) or external B2B services for supporting those use cases.


Comment 4.5
---------------------
The description structure for Fig. 3 can be improved. For example, use case ontology, prompt engineering, LLMs, UI/UX, regular database and vector database are shared by all phases and might not be scoped under network service provider initialisation.

Reply 4.5
---------------------
We have revised Fig. 3 containing three phases now without duplicate or misplaced symbols. We hope the new diagram is clearer in illustrating the operations of both network service providers (green) and use case innovators (blue) for our readers.



==> reviewer_comments_2nd_round.tex <==
Automatic Retrieval-augmented Generation of 6G Network Specifications for Use Case
[IEEE Comm Mag] – Reviewer Comments - 2nd Round

====================================

Reviewer: 1, 2, 3

====================================

Reply:
We thank again all the reviewers for their valuable comments.

====================================

Reviewer: 4

====================================

Comment 4.1
---------------------
Thanks for addressing most of my comments.

Still, I believe that Limitation 3 (Section II, C) needs to be revised. It appears that there is some confusion between the lack of up-to-date training data and the lack of up-to-date design references for xApp or rApp. As the paper addresses the latter, the text should be adjusted accordingly to minimize confusion.

Reply 4.1
---------------------
Dear reviewer, thank you for the suggestion. After changing the wording, we found the clarity is indeed improved. (see revised Section II.C Limitation 3).

